A Measurement of the Millimeter Emission and the Sunyaev-Zel'dovich Effect Associated with Low-Frequency Radio Sources

We present a statistical analysis of the millimeter-wavelength properties of 1.4 GHz-selected sources and a detection of the Sunyaev-Zel'dovich (SZ) effect associated with the halos that host them. The Atacama Cosmology Telescope (ACT) has conducted a survey at 148 GHz, 218 GHz and 277 GHz along the celestial equator. Using samples of radio sources selected at 1.4 GHz from FIRST and NVSS, we measure the stacked 148, 218 and 277 GHz flux densities for sources with 1.4 GHz flux densities ranging from 5 to 200 mJy. At these flux densities, the radio source population is dominated by active galactic nuclei (AGN), with both steep and flat spectrum populations, which have combined radio-to-millimeter spectral indices ranging from 0.5 to 0.95, reflecting the prevalence of steep spectrum sources at high flux densities and the presence of flat spectrum sources at lower flux densities. The thermal SZ effect associated with the halos that host the AGN is detected at the 5$\sigma$ level through its spectral signature. When we compare the SZ effect with weak lensing measurements of radio galaxies, we find that the relation between the two is consistent with that measured by Planck for local bright galaxies. We present a detection of the SZ effect in some of the lowest mass halos (average $M_{200}\approx10^{13}$M$_{\odot}h_{70}^{-1}$) studied to date. This detection is particularly important in the context of galaxy evolution models, as it confirms that galaxies with radio AGN also typically support hot gaseous halos. With Herschel observations, we show that the SZ detection is not significantly contaminated by dust. We show that 5 mJy$<S_{1.4}<$200 mJy radio sources contribute $\ell(\ell+1)C_{\ell}/(2\pi)=0.37\pm0.03\mu$K$^2$ to the angular power spectrum at $\ell=3000$ at 148 GHz, after accounting for the SZ effect associated with their host halos.

==> arxiv update/numbers.tex <==
%% ---------- ACT Data ----------
\newcommand{\AROnePixwin}{1.06}
\newcommand{\ARTwoPixwin}{1.10}
\newcommand{\ARThreePixwin}{1.14}

%% ---------- CROSS Matched Catalog ----------
%%%% Stacking Results
\newcommand{\TotalInRegionSources}{9,436}
\newcommand{\TotalInFluxRangeSources}{4,563}
\newcommand{\ACTExcluded}{219}
\newcommand{\ACTExcludedPercent}{4.8\%}
\newcommand{\TotalStackedSources}{4,344}
\newcommand{\SourcesWithIR}{2,123}
\newcommand{\NullChiSqAROne}{5.7}
\newcommand{\NullDOFAROne}{7}
\newcommand{\NullPTEAROne}{0.57}
\newcommand{\NullChiSqARTwo}{11.3}
\newcommand{\NullDOFARTwo}{7}
\newcommand{\NullPTEARTwo}{0.13}
\newcommand{\NullChiSqARThree}{3.4}
\newcommand{\NullDOFARThree}{7}
\newcommand{\NullPTEARThree}{0.85}
\newcommand{\NBins}{7}
\newcommand{\ParASZWithSZSignif}{5}
\newcommand{\FinalModelDir}{plots}

%%%% Binning Info
\newcommand{\LowBinCount}{1,767}
\newcommand{\HiBinCount}{61}
\newcommand{\LowBinFlux}{6.4}
\newcommand{\HiBinFlux}{149.1}

%%%% Standard model with SZ and no SFGs
\newcommand{\SPivmJy}{149.1}
\newcommand{\ModelChiSqWithSZ}{31.1}
\newcommand{\ModelDOFWithSZ}{27}
\newcommand{\ModelPTEWithSZ}{0.27}
\newcommand{\ParASZWithSZ}{$0.306 \pm 0.052$}
\newcommand{\ParAlphaWithSZ}{$0.95 \pm 0.01$}
\newcommand{\ParBetaWithSZ}{$0.31 \pm 0.02$}
\newcommand{\ParLBolWithSZ}{$9.96 \pm 0.08$}

%%%% Model with SZ, steepening and no SFGs
\newcommand{\ModelChiSqWithSZandSteep}{31.0}
\newcommand{\ModelDOFWithSZandSteep}{25}
\newcommand{\ModelPTEWithSZandSteep}{0.19}
\newcommand{\ParSWithSZandSteep}{$1.05 \pm 0.30$}
\newcommand{\ParASZWithSZandSteepSignif}{5}
\newcommand{\ParASZWithSZandSteep}{$0.304 \pm 0.057$}
\newcommand{\ParLBolWithSZandSteep}{$9.97 \pm 0.08$}
\newcommand{\ParAlphaWithSZandSteep}{$0.94 \pm 0.02$}
\newcommand{\ParBetaWithSZandSteep}{$0.31 \pm 0.02$}

%%%% Model with no SZ and no SFGs but with steepening
\newcommand{\ModelChiSqWithoutSZandSteep}{55.3}
\newcommand{\ModelDOFWithoutSZandSteep}{26}
\newcommand{\ModelPTEWithoutSZandSteep}{$7 \times 10^{-4}$}
\newcommand{\ParSWithoutSZandSteep}{$1.29 \pm 0.22$}
\newcommand{\ParLBolWithoutSZandSteep}{$10.10 \pm 0.05$}

%% ---------- GMBCG ----------
\newcommand{\GMBCGInReg}{1,903}
\newcommand{\GMBCGAssocSourcesPreThin}{405}
\newcommand{\GMBCGAssocSourcesPostThin}{192}
\newcommand{\GMBCGFracChangeAROne}{$< 5\%$}
    
%% ---------- Best SFG ----------
\newcommand{\BestSFGCutNum}{211}
    
%% ---------- Y-Scaling ----------
\newcommand{\Rfh}{0.25}
\newcommand{\Tfh}{0.64}
\newcommand{\AROneMeanCorr}{23\%}
\newcommand{\AROneMedCorr}{7\%}
\newcommand{\ARThreeMeanCorr}{37\%}
\newcommand{\ARThreeMedCorr}{10\%}
\newcommand{\AROneMeanCorrFac}{1.23}
\newcommand{\AROneMedCorrFac}{1.07}
\newcommand{\ARThreeMeanCorrFac}{1.37}
\newcommand{\ARThreeMedCorrFac}{1.10}
\newcommand{\AROneToARThreeMeanCorr}{12\%}
\newcommand{\YIntegratedAmpl}{$5.4 \pm 1.2^{stat} \pm 3^{sys} \times 10^{-8}$}
\newcommand{\YIntegratedAmplnosys}{$5.4 \pm 1.2^{stat} \times 10^{-8}$}
\newcommand{\YIntegratedAmplHo}{$4.5 \pm 1.0 \times 10^{-8}$}
\newcommand{\YIntegratedAmplPlanck}{$8.7 \pm 2.0 \times 10^{-8}$}
\newcommand{\YIntegratedAmplNeto}{$5.7 \pm 1.3 \times 10^{-8}$}

\newcommand{\RfhBest}{0.34}
\newcommand{\TfhBest}{1.24}
\newcommand{\AROneMeanCorrBest}{153\%}
\newcommand{\AROneMedCorrBest}{32\%}
\newcommand{\ARThreeMeanCorrBest}{271\%}
\newcommand{\ARThreeMedCorrBest}{52\%}
\newcommand{\AROneMeanCorrFacBest}{2.53}
\newcommand{\AROneMedCorrFacBest}{1.32}
\newcommand{\ARThreeMeanCorrFacBest}{3.71}
\newcommand{\ARThreeMedCorrFacBest}{1.52}
\newcommand{\AROneToARThreeMedCorrBest}{15\%}
\newcommand{\YIntBest}{$1.4 \pm 0.5^{stat} \pm 0.6 ^{sys} \times 10^{-7}$}
\newcommand{\YIntBestnosys}{$1.4 \pm 0.5^{stat}\times 10^{-7}$}
\newcommand{\YIntBestPlanck}{$2.0 \pm 0.7 \times 10^{-7}$ }
\newcommand{\YIntBestNeto}{$1.5 \pm 0.5 \times 10^{-7}$}


%% ---------- Thinning Cuts ----------
\newcommand{\KimballPercentThin}{35\%}
\newcommand{\BestPercentThin}{1.1\%}
    

==> arxiv update/table.tex <==
 1 & 5.00 -- 8.47 & 1767 &  6.43 &  3.7 $\pm$  0.2 & 0.37 $\pm$ 0.05 & 0.66 $\pm$ 0.08 &  1.0 $\pm$  0.2 & \multirow{7}{*}{ 3.9 $\pm$  0.4} & \multirow{7}{*}{ 4.4 $\pm$  0.4} & \multirow{7}{*}{ 4.4 $\pm$  0.4} \\
 2 & 8.47 -- 14.3 & 1092 &  10.9 &  5.7 $\pm$  0.3 & 0.38 $\pm$ 0.07 & 0.79 $\pm$  0.1 &  1.3 $\pm$  0.2 &  &  &   \\
 3 & 14.3 -- 24.3 & 672 &  18.5 &  7.8 $\pm$  0.3 & 0.59 $\pm$ 0.09 & 0.83 $\pm$  0.1 &  1.5 $\pm$  0.3 &  &  &   \\
 4 & 24.3 -- 41.2 & 412 &  31.3 &  12. $\pm$  0.5 & 0.64 $\pm$  0.1 &  1.1 $\pm$  0.2 & 0.96 $\pm$  0.3 &  &  &   \\
 5 & 41.2 -- 69.7 & 222 &  53.5 &  21. $\pm$  0.9 & 0.94 $\pm$  0.1 &  1.4 $\pm$  0.2 &  1.5 $\pm$  0.5 &  &  &   \\
 6 & 69.7 -- 118. & 118 &  88.4 &  30. $\pm$   1. &  1.4 $\pm$  0.2 &  1.8 $\pm$  0.3 &  2.7 $\pm$  0.7 &  &  &   \\
 7 & 118. -- 200. & 61 &  149. &  45. $\pm$   1. &  1.9 $\pm$  0.3 & 0.83 $\pm$  0.4 &  1.5 $\pm$  0.9 &  &  &   \\

